Towards Evaluating the Robustness of Visual State Space Models

Vision State Space Models (VSSMs), a novel architecture that combines the strengths of recurrent neural networks and latent variable models, have demonstrated remarkable performance in visual perception tasks by efficiently capturing long-range dependencies and modeling complex visual dynamics. However, their robustness under natural and adversarial perturbations remains a critical concern. In this work, we present a comprehensive evaluation of VSSMs' robustness under various perturbation scenarios, including occlusions, image structure, common corruptions, and adversarial attacks, and compare their performance to well-established architectures such as transformers and Convolutional Neural Networks. Furthermore, we investigate the resilience of VSSMs to object-background compositional changes on sophisticated benchmarks designed to test model performance in complex visual scenes. We also assess their robustness on object detection and segmentation tasks using corrupted datasets that mimic real-world scenarios. To gain a deeper understanding of VSSMs' adversarial robustness, we conduct a frequency-based analysis of adversarial attacks, evaluating their performance against low-frequency and high-frequency perturbations. Our findings highlight the strengths and limitations of VSSMs in handling complex visual corruptions, offering valuable insights for future research. Our code and models will be available at https://github.com/HashmatShadab/MambaRobustness.

==> tables/coco_dc_small.tex <==
\begin{table*}[t]
\caption{\small Average Precision (AP) scores for different architectures on the COCO-DC dataset~\cite{malik2024objectcompose}, detailing results for small (APs), medium (APm), and large objects (APl).}
\label{tab:coco_dc}
\setlength{\tabcolsep}{6.0pt}
\definecolor{lightblue}{HTML}{E6F5FF}
\definecolor{lightgreen}{HTML}{E6FFE6}
\definecolor{lightyellow}{HTML}{FFFFE6}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cccc}
\toprule
\rowcolor{LightCyan}
\textbf{Model} & \textbf{Original} & \textbf{Color} & \textbf{Texture} & \textbf{Average}  \\ \midrule
\cellcolor{gray!15}\textbf{ConvNext-T} & \cellcolor{gray!5}66.2  & 55.0  & 53.5 & 54.25 \dec{11.95}\\
\cellcolor{gray!15}\textbf{Swin-T} & \cellcolor{gray!5}66.3 &55.1 & 53.6&  54.35\dec{11.95} \\
\cellcolor{gray!15}\textbf{Swin-S} & \cellcolor{gray!5}69.1& 57.4& 56.0& 56.70\dec{12.40} \\
\cellcolor{gray!15}\textbf{VMamba-T} & \cellcolor{gray!5}69.3&56.2& 53.2& 54.57\dec{14.73}  \\
\cellcolor{gray!15}\textbf{VMamba-S} & \cellcolor{gray!5}70.9& 56.7& 55.7&  56.20\dec{14.70}\\ \bottomrule
\end{tabular}
}
\vspace{-1em}
\end{table*}


==> tables/ood.tex <==


% \begin{table}[t]
%     \caption{\textnormal{\textbf{Comparison in domain generalization setting. Models trained on ImageNet are evaluated on datasets with domain shifts.} } }
%     \small \centering
%  \setlength{\tabcolsep}{4pt}
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{|l |c|cccc|l|}
%     \toprule
%     % & \multicolumn{5}{c}{\textbf{Target Datasets}} \\ \cmidrule(lr){2-6}
%     \rowcolor{LightCyan} 
%     Model \downarrow & ImageNet & ImageNet V2 & ImageNet Sketch & ImageNet A &  ImageNet R  & Average\\
%     \midrule
%     \cellcolor{gray!15}ConvNext-T  &  \cellcolor{gray!5}84.01 & 75.45\dec{08.56} & 39.34\dec{44.67} & 21.03\dec{62.98} & 36.99\dec{47.02} & 43.20\dec{40.81} \\
%     \cellcolor{gray!15}ViT-T& \cellcolor{gray!5}75.35 & 63.05\dec{12.30} & 20.88\dec{54.47} & 3.31\dec{72.04} & 20.29\dec{55.06} & 26.88\dec{44.47} \\
%     \cellcolor{gray!15}Swin-T  & \cellcolor{gray!5}80.91 & 69.31\dec{11.60} & 29.24\dec{51.67} & 8.93\dec{71.98} & 28.52\dec{52.39} & 34.00\dec{46.91} \\
%     \cellcolor{gray!15}VSSM-T\emph{(v0)} & \cellcolor{gray!5}81.92 & 70.82\dec{11.10} & 33.01\dec{48.91} & 13.56\dec{68.36} & 32.11\dec{49.81} & 37.37\dec{44.55} \\
%     \cellcolor{gray!15}VSSM-T\emph{(v2)} & \cellcolor{gray!5}82.28 & 71.16\dec{11.12} & 33.99\dec{48.29} & 12.08\dec{70.20} & 32.05\dec{50.23} & 37.32\dec{44.96} \\
%     \midrule
%      \cellcolor{gray!15}ConvNext-S & \cellcolor{gray!5}84.86 & 74.89\dec{9.97} & 43.63\dec{41.23} & 29.20\dec{55.66} & 41.27\dec{43.59} & 47.25\dec{37.61} \\
%     \cellcolor{gray!15}ViT-S & \cellcolor{gray!5}81.40 & 69.98\dec{11.42} & 32.77\dec{48.63} & 13.09\dec{68.31} & 31.14\dec{50.26} & 36.74\dec{44.66} \\
%     \cellcolor{gray!15}Swin-S  & \cellcolor{gray!5}82.90 & 71.62\dec{11.28} & 31.97\dec{50.93} & 15.72\dec{67.29} & 31.93\dec{50.97} & 37.81\dec{45.09} \\
%     \cellcolor{gray!15}VSSM-S\emph{(v0)} & \cellcolor{gray!5}83.15 & 72.89\dec{10.26} & 38.05\dec{45.10} & 17.28\dec{65.87} & 37.05\dec{46.10} & 41.32\dec{41.83} \\
%     \cellcolor{gray!15}VSSM-S\emph{(v2)}  & \cellcolor{gray!5}83.48 & 73.01\dec{10.47} & 36.98\dec{46.50} & 16.45\dec{67.03} & 35.75\dec{47.73} & 40.55\dec{42.93} \\
%     \midrule
%      \cellcolor{gray!15}ConvNext-B & \cellcolor{gray!5}85.52 & 75.45\dec{10.07} & 48.62\dec{36.90} & 30.45\dec{55.07} & 46.08\dec{39.44} & 50.15\dec{35.37} \\
%     \cellcolor{gray!15}ViT-B & \cellcolor{gray!5}84.40 & 73.84\dec{10.56} & 43.01\dec{41.39} & 24.09\dec{60.31} & 41.03\dec{43.37} & 45.49\dec{38.91} \\
%     \cellcolor{gray!15}Swin-B  & \cellcolor{gray!5}84.71 & 74.74\dec{09.97} & 45.07\dec{39.64} & 27.53\dec{27.18} & 43.84\dec{40.87} & 47.79\dec{36.92} \\
%     \cellcolor{gray!15}VSSM-B\emph{(v0)}  & \cellcolor{gray!5}83.48 & 72.97\dec{10.51} & 38.24\dec{45.24} & 18.88\dec{64.60} & 37.33\dec{46.15} & 41.86\dec{41.62} \\
%     \cellcolor{gray!15}VSSM-B\emph{(v2)}  & \cellcolor{gray!5}83.76 & 73.22\dec{10.54} & 38.53\dec{45.23} & 18.35\dec{65.41} & 35.99\dec{47.77} & 41.52\dec{42.24} \\

    
%     \bottomrule
%     \end{tabular}}
%     \label{tab:robustness}
%     \vspace{-1em}
% \end{table}

% \begin{table}[t]
%  \centering
%     \caption{\small Comparison in domain generalization setting. Models trained on ImageNet are evaluated on datasets with domain shifts.} 
%         \label{tab:robustness}

%  \setlength{\tabcolsep}{10.0pt}
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{|l |c|cccc|l|}
%     \toprule
%     % & \multicolumn{5}{c}{\textbf{Target Datasets}} \\ \cmidrule(lr){2-6}
%     % \rowcolor{LightCyan}
%     \small{Model} \downarrow & ImageNet & ImageNetV2 & ImageNet-S & ImageNet-A &  ImageNet-R  & Average\\
%     \midrule
%      \cellcolor{gray!15}ConvNext-T  &  \cellcolor{gray!5}81.87 & 70.67\dec{08.56} & 33.96\dec{44.67} & 10.48\dec{62.98} & 32.53\dec{47.02} & 43.20\dec{40.81} \\
%     \cellcolor{gray!15}ConvNext-T*  &  \cellcolor{gray!5}84.01 & 73.68\dec{08.56} & 39.34\dec{44.67} & 21.03\dec{62.98} & 36.99\dec{47.02} & 43.20\dec{40.81} \\
%     \cellcolor{gray!15}ViT-T& \cellcolor{gray!5}75.35 & 63.05\dec{12.30} & 20.88\dec{54.47} & 3.31\dec{72.04} & 20.29\dec{55.06} & 26.88\dec{44.47} \\
%     \cellcolor{gray!15}Swin-T  & \cellcolor{gray!5}80.91 & 69.31\dec{11.60} & 29.24\dec{51.67} & 8.93\dec{71.98} & 28.52\dec{52.39} & 34.00\dec{46.91} \\
%     \cellcolor{gray!15}VSSM-T & \cellcolor{gray!5}82.28 & 71.16\dec{11.12} & 33.99\dec{48.29} & 12.08\dec{70.20} & 32.05\dec{50.23} & 37.32\dec{44.96} \\
%     \midrule
%      \cellcolor{gray!15}ConvNext-S & \cellcolor{gray!5}82.82 & 72.07\dec{9.97} & 37.16\dec{41.23} & 14.43\dec{55.66} & 35.57\dec{43.59} & 47.25\dec{37.61} \\
%      \cellcolor{gray!15}ConvNext-S* & \cellcolor{gray!5}84.86 & 74.89\dec{9.97} & 43.63\dec{41.23} & 29.20\dec{55.66} & 41.27\dec{43.59} & 47.25\dec{37.61} \\
%     \cellcolor{gray!15}ViT-S & \cellcolor{gray!5}81.40 & 69.98\dec{11.42} & 32.77\dec{48.63} & 13.09\dec{68.31} & 31.14\dec{50.26} & 36.74\dec{44.66} \\
%     \cellcolor{gray!15}Swin-S  & \cellcolor{gray!5}82.90 & 71.62\dec{11.28} & 31.97\dec{50.93} & 15.72\dec{67.29} & 31.93\dec{50.97} & 37.81\dec{45.09} \\
%     \cellcolor{gray!15}VSSM-S  & \cellcolor{gray!5}83.48 & 73.01\dec{10.47} & 36.98\dec{46.50} & 16.45\dec{67.03} & 35.75\dec{47.73} & 40.55\dec{42.93} \\
%     \midrule
%     \cellcolor{gray!15}ConvNext-B & \cellcolor{gray!5}83.75 & 73.68\dec{10.07} & 38.23\dec{36.90} & 18.16\dec{55.07} & 36.66\dec{39.44} & 50.15\dec{35.37} \\
%      \cellcolor{gray!15}ConvNext-B* & \cellcolor{gray!5}85.52 & 75.45\dec{10.07} & 48.62\dec{36.90} & 30.45\dec{55.07} & 46.08\dec{39.44} & 50.15\dec{35.37} \\
%     \cellcolor{gray!15}ViT-B & \cellcolor{gray!5}84.40 & 73.84\dec{10.56} & 43.01\dec{41.39} & 24.09\dec{60.31} & 41.03\dec{43.37} & 45.49\dec{38.91} \\

%            \cellcolor{gray!15}Swin-B  & \cellcolor{gray!5}83.08 & 72.09\dec{10.99} & 32.62\dec{50.46} & 17.95\dec{65.13} & 33.23\dec{49.85} & 38.97\dec{44.11} \\
%     % \cellcolor{gray!15}Swin-B*  & \cellcolor{gray!5}84.71 & 74.74\dec{09.97} & 45.07\dec{39.64} & 27.53\dec{27.18} & 43.84\dec{40.87} & 47.79\dec{36.92} \\
%     \cellcolor{gray!15}VSSM-B  & \cellcolor{gray!5}83.76 & 73.22\dec{10.54} & 38.53\dec{45.23} & 18.35\dec{65.41} & 35.99\dec{47.77} & 41.52\dec{42.24} \\

    
%     \bottomrule
%     \end{tabular}}
% \end{table}


% \begin{table*}[t]
%  \centering
%     \caption{\small Top-1 classification accuracy for the domain generalization setting across various architectures and datasets. Models trained on ImageNet are evaluated on datasets with domain shifts.} 
%         \label{tab:robustness_full}
%     \small
%  \setlength{\tabcolsep}{16.0pt}
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{|l|c|cccc|l|}
%     \toprule
%     \rowcolor{LightCyan}
%     Model $\downarrow$ & ImageNet & ImageNetV2 & ImageNet-S & ImageNet-A &  ImageNet-R  & Average\\
%     \midrule
%      \cellcolor{gray!15}ConvNext-T  &  \cellcolor{gray!5}81.87 & 70.67\dec{11.20} & 33.96\dec{47.91} & 10.48\dec{71.39} & 32.53\dec{49.34} & 36.90\dec{44.97} \\
%     \cellcolor{gray!15}ViT-T& \cellcolor{gray!5}75.35 & 63.05\dec{12.30} & 20.88\dec{54.47} & 3.31\dec{72.04} & 20.29\dec{55.06} & 26.88\dec{48.47} \\
%     \cellcolor{gray!15}Swin-T  & \cellcolor{gray!5}80.91 & 69.31\dec{11.60} & 29.24\dec{51.67} & 8.93\dec{71.98} & 28.52\dec{52.39} & 34.00\dec{46.91} \\
%     \cellcolor{gray!15}VMamba-T & \cellcolor{gray!5}82.28 & 71.16\dec{11.12} & 33.99\dec{48.29} & 12.08\dec{70.20} & 32.05\dec{50.23} & 37.32\dec{44.96} \\
%      \cellcolor{gray!15}MambaVision-T & \cellcolor{gray!5}82.10 & 71.50\dec{10.60} & 33.49\dec{48.61} & 13.39\dec{68.71} & 32.28\dec{49.82} & 37.66\dec{44.44} \\
%     \midrule
%      \cellcolor{gray!15}ConvNext-S & \cellcolor{gray!5}82.82 & 72.07\dec{10.75} & 37.16\dec{45.66} & 14.43\dec{68.39} & 35.57\dec{47.25} & 39.81\dec{43.01} \\
%     \cellcolor{gray!15}ViT-S & \cellcolor{gray!5}81.40 & 69.98\dec{11.42} & 32.77\dec{48.63} & 13.09\dec{68.31} & 31.14\dec{50.26} & 36.74\dec{44.66} \\
%     \cellcolor{gray!15}Swin-S  & \cellcolor{gray!5}82.90 & 71.62\dec{11.28} & 31.97\dec{50.93} & 15.72\dec{67.18} & 31.93\dec{50.97} & 37.81\dec{45.09} \\
%     \cellcolor{gray!15}VMamba-S  & \cellcolor{gray!5}83.48 & 73.01\dec{10.47} & 36.98\dec{46.50} & 16.45\dec{67.03} & 35.75\dec{47.73} & 40.55\dec{42.93} \\
%     \cellcolor{gray!15}MambaVision-S & \cellcolor{gray!5}83.22 & 72.62\dec{10.60} & 35.53\dec{47.69} & 15.97\dec{67.25} & 33.96\dec{49.26} & 39.52\dec{43.70} \\
%     \midrule
%     \cellcolor{gray!15}ConvNext-B & \cellcolor{gray!5}83.75 & 73.68\dec{10.07} & 38.23\dec{45.52} & 18.16\dec{65.59} & 36.66\dec{47.09} & 41.68\dec{42.07} \\
%     \cellcolor{gray!15}ViT-B & \cellcolor{gray!5}84.40 & 73.84\dec{10.56} & 43.01\dec{41.39} & 24.09\dec{60.31} & 41.03\dec{43.37} & 45.49\dec{38.91} \\
%     \cellcolor{gray!15}Swin-B  & \cellcolor{gray!5}83.08 & 72.09\dec{10.99} & 32.62\dec{50.46} & 17.95\dec{65.13} & 33.23\dec{49.85} & 38.97\dec{44.11} \\
%     \cellcolor{gray!15}VMamba-B  & \cellcolor{gray!5}83.76 & 73.22\dec{10.54} & 38.53\dec{45.23} & 18.35\dec{65.41} & 35.99\dec{47.77} & 41.52\dec{42.24} \\
%             \cellcolor{gray!15}MambaVision-B & \cellcolor{gray!5}83.96 & 73.84\dec{10.12} & 36.69\dec{47.27} & 21.69\dec{62.27} & 35.72\dec{48.24} & 41.98\dec{41.98} \\

%     \bottomrule
%     \end{tabular}}
% \end{table*}




==> tables/shuffle_drop.tex <==
\begin{table}[]
\centering
\caption{Figure 4 (left)}
\setlength{\tabcolsep}{2.0pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{c c c c c c c c c c c c c}
\rotatebox{45}{\scriptsize ResNet-50} & \rotatebox{45}{\scriptsize ConvNext-T} & \rotatebox{45}{\scriptsize ConvNext-S} & \rotatebox{45}{\scriptsize ConvNext-B} & \rotatebox{45}{\scriptsize ViT-T} & \rotatebox{45}{\scriptsize ViT-S} & \rotatebox{45}{\scriptsize ViT-B} & \rotatebox{45}{\scriptsize VSSM-T} & \rotatebox{45}{\scriptsize VSSM-S} & \rotatebox{45}{\scriptsize VSSM-B} & \rotatebox{45}{\scriptsize Swin-T} & \rotatebox{45}{\scriptsize Swin-S} & \rotatebox{45}{\scriptsize Swin-B*} \\
\hline

\heatmapcolor{90.79} & \heatmapcolor{95.98}  & \heatmapcolor{96.24}  & \heatmapcolor{96.96}  & \heatmapcolor{85.71}  & \heatmapcolor{92.88}  & \heatmapcolor{95.18}  & \heatmapcolor{95.75}  & \heatmapcolor{96.73}  & \heatmapcolor{96.88}  & \heatmapcolor{95.41}  & \heatmapcolor{96.05} & \heatmapcolor{96.24}  \\
\hline

\heatmapcolor{82.01}  & \heatmapcolor{94.50}  & \heatmapcolor{94.85}  & \heatmapcolor{95.29}  & \heatmapcolor{78.67}  & \heatmapcolor{88.81}  & \heatmapcolor{92.55}  & \heatmapcolor{94.66}  & \heatmapcolor{95.75}  & \heatmapcolor{96.12}  & \heatmapcolor{93.99}  & \heatmapcolor{94.55}  & \heatmapcolor{95.01}   \\
\hline

\heatmapcolor{67.09}  & \heatmapcolor{91.49}  & \heatmapcolor{91.97}  & \heatmapcolor{91.42}  & \heatmapcolor{67.95}  & \heatmapcolor{81.22}  & \heatmapcolor{87.88}  & \heatmapcolor{91.65}  & \heatmapcolor{93.26}  & \heatmapcolor{94.27}  & \heatmapcolor{90.69}  & \heatmapcolor{91.93}  & \heatmapcolor{91.84}   \\
\hline

\heatmapcolor{33.34}  & \heatmapcolor{83.87}  & \heatmapcolor{82.50}  & \heatmapcolor{78.57}  & \heatmapcolor{42.65}  & \heatmapcolor{63.97}  & \heatmapcolor{75.68}  & \heatmapcolor{85.34}  & \heatmapcolor{87.10}  & \heatmapcolor{90.08}  & \heatmapcolor{85.01}  & \heatmapcolor{86.33}  & \heatmapcolor{85.62}  \\
\hline

\heatmapcolor{10.93}  & \heatmapcolor{70.95} & \heatmapcolor{60.54} & \heatmapcolor{58.91}  & \heatmapcolor{19.05}  & \heatmapcolor{45.21}  & \heatmapcolor{55.52}  & \heatmapcolor{73.72}  & \heatmapcolor{73.68}  & \heatmapcolor{80.79} & \heatmapcolor{76.60}  & \heatmapcolor{75.46} & \heatmapcolor{73.29}    \\
\hline
\heatmapcolor{1.07}  & \heatmapcolor{18.61} & \heatmapcolor{11.51} & \heatmapcolor{6.43}  & \heatmapcolor{1.00}  & \heatmapcolor{3.14}  & \heatmapcolor{5.00}  & \heatmapcolor{15.45}  & \heatmapcolor{13.83}  & \heatmapcolor{22.50} & \heatmapcolor{25.79}  & \heatmapcolor{12.83} & \heatmapcolor{17.17}    \\
\hline


\end{tabular}
}
\end{table}


==> tables/transferability.tex <==


% \begin{table}[t]
% \centering
% \caption{\small Robust accuracy of models under white-box and black-box settings for FGSM and PGD attacks.}
% \label{tab:adv_transf_main}
% \setlength{\tabcolsep}{2.0pt}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{|l| c c c c c c c c c c c c c|}
% \hline
% \rowcolor{LightCyan}
% & \rotatebox{0}{\scriptsize \textbf{VSSM-T}} & \rotatebox{0}{\scriptsize \textbf{VSSM-S}} & \rotatebox{0}{\scriptsize \textbf{VSSM-B}} & \rotatebox{0}{\scriptsize \textbf{ResNet-50}} & \rotatebox{0}{\scriptsize \textbf{ConvNext-T}} & \rotatebox{0}{\scriptsize \textbf{ConvNext-S}} & \rotatebox{0}{\scriptsize \textbf{ConvNext-B}} & \rotatebox{0}{\scriptsize \textbf{ViT-T}} & \rotatebox{0}{\scriptsize \textbf{ViT-S}} & \rotatebox{0}{\scriptsize \textbf{ViT-B}} & \rotatebox{0}{\scriptsize \textbf{Swin-T}} & \rotatebox{0}{\scriptsize \textbf{Swin-S}} & \rotatebox{0}{\scriptsize \textbf{Swin-B*}} \\
% \hline
% \rowcolor{gray!5}
% \multicolumn{14}{|c|}{Fast Gradient Sign Method (FGSM) at $\epsilon=\frac{8}{255}$ } \\
% \hline
% {\scriptsize VSSM-T} &   \heatmapcolor{42.90}  & \heatmapcolor{66.34}  & \heatmapcolor{65.10}  & \heatmapcolor{80.20}  & \heatmapcolor{73.72}  & \heatmapcolor{78.60}  & \heatmapcolor{78.90}  & \heatmapcolor{79.46}  & \heatmapcolor{83.64}  & \heatmapcolor{86.94}  & \heatmapcolor{72.22} & \heatmapcolor{76.38} & \heatmapcolor{81.46}    \\
% \hline
% {\scriptsize VSSM-S} &  \heatmapcolor{62.24}  & \heatmapcolor{48.42}  & \heatmapcolor{63.00}  & \heatmapcolor{79.70}  & \heatmapcolor{72.46}  & \heatmapcolor{76.56}  & \heatmapcolor{75.66}  & \heatmapcolor{78.42}  & \heatmapcolor{81.56}  & \heatmapcolor{84.58}  & \heatmapcolor{70.96}  & \heatmapcolor{72.92}  & \heatmapcolor{78.20}   \\
% \hline
% {\scriptsize VSSM-B} &   \heatmapcolor{65.52}  & \heatmapcolor{66.96}  & \heatmapcolor{51.24}  & \heatmapcolor{81.22}  & \heatmapcolor{74.28}  & \heatmapcolor{77.86}  & \heatmapcolor{77.38}  & \heatmapcolor{79.12}  & \heatmapcolor{83.62}  & \heatmapcolor{86.24}  & \heatmapcolor{73.24}  & \heatmapcolor{76.30}  & \heatmapcolor{80.74} \\
% \hline
% {\scriptsize ResNet-50} &   \heatmapcolor{81.38}  & \heatmapcolor{83.24}  & \heatmapcolor{83.84}  & \heatmapcolor{30.46}  & \heatmapcolor{81.98}  & \heatmapcolor{86.46}  & \heatmapcolor{87.12}  & \heatmapcolor{75.94}  & \heatmapcolor{84.74}  & \heatmapcolor{89.12}  & \heatmapcolor{80.64}  & \heatmapcolor{85.00} & \heatmapcolor{88.36}  \\
% \hline
% {\scriptsize ConvNext-T} &  \heatmapcolor{72.78} & \heatmapcolor{75.20} & \heatmapcolor{74.26}  & \heatmapcolor{81.84}  & \heatmapcolor{37.14}  & \heatmapcolor{68.14}  & \heatmapcolor{69.96}  & \heatmapcolor{78.86}  & \heatmapcolor{82.56} & \heatmapcolor{84.96}  & \heatmapcolor{71.86} & \heatmapcolor{76.60}   & \heatmapcolor{77.24}  \\
% \hline
% {\scriptsize ConvNext-S} &  \heatmapcolor{81.16} & \heatmapcolor{82.92} & \heatmapcolor{81.66}  & \heatmapcolor{86.14}  & \heatmapcolor{74.40}  & \heatmapcolor{54.28}  & \heatmapcolor{75.12}  & \heatmapcolor{82.44}  & \heatmapcolor{85.74} & \heatmapcolor{87.20}  & \heatmapcolor{79.32} & \heatmapcolor{82.40}  & \heatmapcolor{81.10}  \\
% \hline
% {\scriptsize ConvNext-B} &  \heatmapcolor{75.94} & \heatmapcolor{76.80} & \heatmapcolor{76.18}  & \heatmapcolor{83.26}  & \heatmapcolor{68.98}  & \heatmapcolor{69.30}  & \heatmapcolor{45.42}  & \heatmapcolor{79.02}  & \heatmapcolor{82.36} & \heatmapcolor{83.74}  & \heatmapcolor{75.60} & \heatmapcolor{76.80}  & \heatmapcolor{75.76}   \\
% \hline
% {\scriptsize ViT-T} &   \heatmapcolor{85.92} & \heatmapcolor{88.30} & \heatmapcolor{88.88}  & \heatmapcolor{82.68}  & \heatmapcolor{84.62}  & \heatmapcolor{86.78}  & \heatmapcolor{88.26}  & \heatmapcolor{2.28}  & \heatmapcolor{50.04} & \heatmapcolor{69.90}  & \heatmapcolor{75.66} & \heatmapcolor{79.72}  & \heatmapcolor{83.84}  \\
% \hline
% {\scriptsize ViT-S} &    \heatmapcolor{81.74} & \heatmapcolor{83.76} & \heatmapcolor{84.46}  & \heatmapcolor{81.70}  & \heatmapcolor{79.92}  & \heatmapcolor{82.82}  & \heatmapcolor{84.02}  & \heatmapcolor{45.40}  & \heatmapcolor{11.02} & \heatmapcolor{54.82}  & \heatmapcolor{72.50} & \heatmapcolor{75.98} & \heatmapcolor{75.08}  \\
% \hline
% {\scriptsize ViT-B} &    \heatmapcolor{82.46} & \heatmapcolor{84.02} & \heatmapcolor{84.48}  & \heatmapcolor{81.90}  & \heatmapcolor{79.70}  & \heatmapcolor{81.04}  & \heatmapcolor{82.04}  & \heatmapcolor{58.50}  & \heatmapcolor{53.84} & \heatmapcolor{24.24}  & \heatmapcolor{75.82} & \heatmapcolor{77.62}  & \heatmapcolor{75.58} \\
% \hline
% {\scriptsize Swin-T} &    \heatmapcolor{72.40} & \heatmapcolor{76.06} & \heatmapcolor{75.58}  & \heatmapcolor{82.82}  & \heatmapcolor{73.62}  & \heatmapcolor{77.46}  & \heatmapcolor{79.28}  & \heatmapcolor{76.48}  & \heatmapcolor{80.66} & \heatmapcolor{85.46}  & \heatmapcolor{28.86} & \heatmapcolor{56.22}  & \heatmapcolor{68.34}  \\
% \hline
% {\scriptsize Swin-S} &   \heatmapcolor{78.24} & \heatmapcolor{79.10} & \heatmapcolor{79.30}  & \heatmapcolor{85.46}  & \heatmapcolor{78.56}  & \heatmapcolor{81.76}  & \heatmapcolor{81.78}  & \heatmapcolor{79.38}  & \heatmapcolor{83.04} & \heatmapcolor{86.58}  & \heatmapcolor{61.94} & \heatmapcolor{48.00}  & \heatmapcolor{70.92} \\
% \hline
% {\scriptsize Swin-B*} &   \heatmapcolor{86.70} & \heatmapcolor{87.72} & \heatmapcolor{87.30}  & \heatmapcolor{89.20}  & \heatmapcolor{82.96}  & \heatmapcolor{84.38}  & \heatmapcolor{84.36}  & \heatmapcolor{82.38}  & \heatmapcolor{85.72} & \heatmapcolor{87.86}  & \heatmapcolor{75.62} & \heatmapcolor{77.38}  & \heatmapcolor{57.24} \\
% \hline

% \rowcolor{gray!5}
% \multicolumn{14}{|c|}{Projected Gradient Decent (PGD) at $\epsilon=\frac{8}{255}$} \\
% \hline
% {\scriptsize VSSM-T} &   \heatmapcolor{0.00}  & \heatmapcolor{37.26}  & \heatmapcolor{35.56}  & \heatmapcolor{81.44}  & \heatmapcolor{64.98}  & \heatmapcolor{76.84}  & \heatmapcolor{75.48}  & \heatmapcolor{82.58}  & \heatmapcolor{89.16}  & \heatmapcolor{91.80}  & \heatmapcolor{65.76} & \heatmapcolor{74.72} & \heatmapcolor{83.02}  \\
% \hline
% {\scriptsize VSSM-S} & \heatmapcolor{16.88} & \heatmapcolor{0.02} & \heatmapcolor{23.94} & \heatmapcolor{77.54} & \heatmapcolor{55.76} & \heatmapcolor{68.78} & \heatmapcolor{65.98} &\heatmapcolor{79.26} & \heatmapcolor{86.06} & \heatmapcolor{89.42} & \heatmapcolor{58.92} & \heatmapcolor{65.92} & \heatmapcolor{76.16}   \\
% \hline
% {\scriptsize VSSM-B} & \heatmapcolor{15.98} & \heatmapcolor{25.26} & \heatmapcolor{0.00} & \heatmapcolor{77.38} & \heatmapcolor{54.42} & \heatmapcolor{68.58} & \heatmapcolor{65.24} & \heatmapcolor{79.76} & \heatmapcolor{86.24} & \heatmapcolor{89.94} & \heatmapcolor{57.40} & \heatmapcolor{66.52} & \heatmapcolor{77.26}   \\
% \hline
% {\scriptsize ResNet-50} & \heatmapcolor{83.34} & \heatmapcolor{86.98} & \heatmapcolor{87.04} & \heatmapcolor{0.00} & \heatmapcolor{85.54} & \heatmapcolor{90.46} & \heatmapcolor{89.28} & \heatmapcolor{82.48} & \heatmapcolor{89.96} & \heatmapcolor{93.18} & \heatmapcolor{84.18} &\heatmapcolor{89.24} &\heatmapcolor{92.16}   \\
% \hline
% {\scriptsize ConvNext-T} &  \heatmapcolor{73.74} & \heatmapcolor{78.36} & \heatmapcolor{76.62}  & \heatmapcolor{84.98}  & \heatmapcolor{0.00}  & \heatmapcolor{59.56}  & \heatmapcolor{67.00}  & \heatmapcolor{83.26}  & \heatmapcolor{88.06} & \heatmapcolor{91.48}  & \heatmapcolor{71.70} & \heatmapcolor{79.46}   & \heatmapcolor{82.32}  \\
% \hline
% {\scriptsize ConvNext-S} &  \heatmapcolor{81.88} & \heatmapcolor{84.78} & \heatmapcolor{84.20}  & \heatmapcolor{88.42}  & \heatmapcolor{59.94}  & \heatmapcolor{0.00}  & \heatmapcolor{69.08}  & \heatmapcolor{84.94}  & \heatmapcolor{90.10} & \heatmapcolor{92.62}  & \heatmapcolor{77.08} & \heatmapcolor{83.00}  & \heatmapcolor{82.92}   \\
% \hline
% {\scriptsize ConvNext-B} &  \heatmapcolor{69.56} & \heatmapcolor{73.62} & \heatmapcolor{72.22}  & \heatmapcolor{83.80}  & \heatmapcolor{50.48}  & \heatmapcolor{53.26}  & \heatmapcolor{0.00}  & \heatmapcolor{81.80}  & \heatmapcolor{86.90} & \heatmapcolor{89.58}  & \heatmapcolor{69.70} & \heatmapcolor{73.80}  & \heatmapcolor{72.78}    \\
% \hline
% {\scriptsize ViT-T} &   \heatmapcolor{92.10} & \heatmapcolor{93.82} & \heatmapcolor{94.26}  & \heatmapcolor{88.14}  & \heatmapcolor{91.30}  & \heatmapcolor{92.74}  & \heatmapcolor{92.90}  & \heatmapcolor{0.00}  & \heatmapcolor{55.58} & \heatmapcolor{77.34}  & \heatmapcolor{84.52} & \heatmapcolor{88.16}  & \heatmapcolor{90.46}  \\
% \hline
% {\scriptsize ViT-S} &    \heatmapcolor{87.28} & \heatmapcolor{89.34} & \heatmapcolor{89.70}  & \heatmapcolor{85.96}  & \heatmapcolor{85.66}  & \heatmapcolor{89.06}  & \heatmapcolor{88.48}  & \heatmapcolor{38.16}  & \heatmapcolor{0.00} & \heatmapcolor{48.68}  & \heatmapcolor{76.98} & \heatmapcolor{80.34} & \heatmapcolor{82.48}  \\
% \hline
% {\scriptsize ViT-B} &   \heatmapcolor{86.18} & \heatmapcolor{87.74} & \heatmapcolor{87.72}  & \heatmapcolor{85.04}  & \heatmapcolor{83.72}  & \heatmapcolor{86.64}  & \heatmapcolor{85.84}  & \heatmapcolor{53.50}  & \heatmapcolor{37.48} & \heatmapcolor{0.00}  & \heatmapcolor{77.02} & \heatmapcolor{79.56}  & \heatmapcolor{78.60}  \\
% \hline
% {\scriptsize Swin-T} &   \heatmapcolor{83.10} & \heatmapcolor{87.58} & \heatmapcolor{87.06}  & \heatmapcolor{89.58}  & \heatmapcolor{81.32}  & \heatmapcolor{85.24}  & \heatmapcolor{87.12}  & \heatmapcolor{83.32}  & \heatmapcolor{89.82} & \heatmapcolor{92.80}  & \heatmapcolor{0.00} & \heatmapcolor{39.00}  & \heatmapcolor{67.88}   \\
% \hline
% {\scriptsize Swin-S} &  \heatmapcolor{83.08} & \heatmapcolor{86.28} & \heatmapcolor{86.26}  & \heatmapcolor{89.76}  & \heatmapcolor{82.16}  & \heatmapcolor{85.82}  & \heatmapcolor{85.42}  & \heatmapcolor{82.96}  & \heatmapcolor{88.80} & \heatmapcolor{92.38}  & \heatmapcolor{25.40} & \heatmapcolor{0.00}  & \heatmapcolor{50.88}  \\
% \hline
% {\scriptsize Swin-B*} &   \heatmapcolor{88.26} & \heatmapcolor{90.46} & \heatmapcolor{90.44}  & \heatmapcolor{90.96}  & \heatmapcolor{84.30}  & \heatmapcolor{85.14}  & \heatmapcolor{85.08}  & \heatmapcolor{84.70}  & \heatmapcolor{89.22} & \heatmapcolor{91.78}  & \heatmapcolor{56.66} & \heatmapcolor{52.68}  & \heatmapcolor{0.08}   \\
% \hline


% \end{tabular}
% }
% \vspace{-1em}

% \end{table}





% \begin{table}[t]
% \centering
% \caption{\small Robust accuracy of models under white-box and black-box settings for FGSM and PGD attacks.}
% \label{tab:adv_transf_main}
% \setlength{\tabcolsep}{2.0pt}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{|l| c c c c c c c c c c c c c|}
% \hline
% \rowcolor{LightCyan}
% & \rotatebox{0}{\scriptsize \textbf{VSSM-T}} & \rotatebox{0}{\scriptsize \textbf{VSSM-S}} & \rotatebox{0}{\scriptsize \textbf{VSSM-B}} & \rotatebox{0}{\scriptsize \textbf{ResNet-50}} & \rotatebox{0}{\scriptsize \textbf{ConvNext-T}} & \rotatebox{0}{\scriptsize \textbf{ConvNext-S}} & \rotatebox{0}{\scriptsize \textbf{ConvNext-B}} & \rotatebox{0}{\scriptsize \textbf{ViT-T}} & \rotatebox{0}{\scriptsize \textbf{ViT-S}} & \rotatebox{0}{\scriptsize \textbf{ViT-B}} & \rotatebox{0}{\scriptsize \textbf{Swin-T}} & \rotatebox{0}{\scriptsize \textbf{Swin-S}} & \rotatebox{0}{\scriptsize \textbf{Swin-B}} \\
% \hline
% \rowcolor{gray!5}
% \multicolumn{14}{|c|}{Fast Gradient Sign Method (FGSM) at $\epsilon=\frac{8}{255}$ } \\
% \hline
% {\scriptsize VSSM-T} &   \heatmapcolor{42.90}  & \heatmapcolor{66.34}  & \heatmapcolor{65.10}  & \heatmapcolor{80.20}  & \heatmapcolor{73.72}  & \heatmapcolor{78.60}  & \heatmapcolor{78.90}  & \heatmapcolor{79.46}  & \heatmapcolor{83.64}  & \heatmapcolor{86.94}  & \heatmapcolor{72.22} & \heatmapcolor{76.38} & \heatmapcolor{74.60}    \\
% \hline
% {\scriptsize VSSM-S} &  \heatmapcolor{62.24}  & \heatmapcolor{48.42}  & \heatmapcolor{63.00}  & \heatmapcolor{79.70}  & \heatmapcolor{72.46}  & \heatmapcolor{76.56}  & \heatmapcolor{75.66}  & \heatmapcolor{78.42}  & \heatmapcolor{81.56}  & \heatmapcolor{84.58}  & \heatmapcolor{70.96}  & \heatmapcolor{72.92}  & \heatmapcolor{71.14}   \\
% \hline
% {\scriptsize VSSM-B} &   \heatmapcolor{65.52}  & \heatmapcolor{66.96}  & \heatmapcolor{51.24}  & \heatmapcolor{81.22}  & \heatmapcolor{74.28}  & \heatmapcolor{77.86}  & \heatmapcolor{77.38}  & \heatmapcolor{79.12}  & \heatmapcolor{83.62}  & \heatmapcolor{86.24}  & \heatmapcolor{73.24}  & \heatmapcolor{76.30}  & \heatmapcolor{73.88} \\
% \hline
% {\scriptsize ResNet-50} &   \heatmapcolor{81.38}  & \heatmapcolor{83.24}  & \heatmapcolor{83.84}  & \heatmapcolor{30.46}  & \heatmapcolor{81.98}  & \heatmapcolor{86.46}  & \heatmapcolor{87.12}  & \heatmapcolor{75.94}  & \heatmapcolor{84.74}  & \heatmapcolor{89.12}  & \heatmapcolor{80.64}  & \heatmapcolor{85.00} & \heatmapcolor{85.42}  \\
% \hline
% {\scriptsize ConvNext-T*} &  \heatmapcolor{72.78} & \heatmapcolor{75.20} & \heatmapcolor{74.26}  & \heatmapcolor{81.84}  & \heatmapcolor{37.14}  & \heatmapcolor{68.14}  & \heatmapcolor{69.96}  & \heatmapcolor{78.86}  & \heatmapcolor{82.56} & \heatmapcolor{84.96}  & \heatmapcolor{71.86} & \heatmapcolor{76.60}   & \heatmapcolor{74.96}  \\
% \hline
% {\scriptsize ConvNext-S*} &  \heatmapcolor{81.16} & \heatmapcolor{82.92} & \heatmapcolor{81.66}  & \heatmapcolor{86.14}  & \heatmapcolor{74.40}  & \heatmapcolor{54.28}  & \heatmapcolor{75.12}  & \heatmapcolor{82.44}  & \heatmapcolor{85.74} & \heatmapcolor{87.20}  & \heatmapcolor{79.32} & \heatmapcolor{82.40}  & \heatmapcolor{80.70}  \\
% \hline
% {\scriptsize ConvNext-B*} &  \heatmapcolor{75.94} & \heatmapcolor{76.80} & \heatmapcolor{76.18}  & \heatmapcolor{83.26}  & \heatmapcolor{68.98}  & \heatmapcolor{69.30}  & \heatmapcolor{45.42}  & \heatmapcolor{79.02}  & \heatmapcolor{82.36} & \heatmapcolor{83.74}  & \heatmapcolor{75.60} & \heatmapcolor{76.80}  & \heatmapcolor{75.82}   \\
% \hline
% {\scriptsize ViT-T} &   \heatmapcolor{85.92} & \heatmapcolor{88.30} & \heatmapcolor{88.88}  & \heatmapcolor{82.68}  & \heatmapcolor{84.62}  & \heatmapcolor{86.78}  & \heatmapcolor{88.26}  & \heatmapcolor{2.28}  & \heatmapcolor{50.04} & \heatmapcolor{69.90}  & \heatmapcolor{75.66} & \heatmapcolor{79.72}  & \heatmapcolor{82.32}  \\
% \hline
% {\scriptsize ViT-S} &    \heatmapcolor{81.74} & \heatmapcolor{83.76} & \heatmapcolor{84.46}  & \heatmapcolor{81.70}  & \heatmapcolor{79.92}  & \heatmapcolor{82.82}  & \heatmapcolor{84.02}  & \heatmapcolor{45.40}  & \heatmapcolor{11.02} & \heatmapcolor{54.82}  & \heatmapcolor{72.50} & \heatmapcolor{75.98} & \heatmapcolor{77.88}  \\
% \hline
% {\scriptsize ViT-B} &    \heatmapcolor{82.46} & \heatmapcolor{84.02} & \heatmapcolor{84.48}  & \heatmapcolor{81.90}  & \heatmapcolor{79.70}  & \heatmapcolor{81.04}  & \heatmapcolor{82.04}  & \heatmapcolor{58.50}  & \heatmapcolor{53.84} & \heatmapcolor{24.24}  & \heatmapcolor{75.82} & \heatmapcolor{77.62}  & \heatmapcolor{78.54} \\
% \hline
% {\scriptsize Swin-T} &    \heatmapcolor{72.40} & \heatmapcolor{76.06} & \heatmapcolor{75.58}  & \heatmapcolor{82.82}  & \heatmapcolor{73.62}  & \heatmapcolor{77.46}  & \heatmapcolor{79.28}  & \heatmapcolor{76.48}  & \heatmapcolor{80.66} & \heatmapcolor{85.46}  & \heatmapcolor{28.86} & \heatmapcolor{56.22}  & \heatmapcolor{55.12}  \\
% \hline
% {\scriptsize Swin-S} &   \heatmapcolor{78.24} & \heatmapcolor{79.10} & \heatmapcolor{79.30}  & \heatmapcolor{85.46}  & \heatmapcolor{78.56}  & \heatmapcolor{81.76}  & \heatmapcolor{81.78}  & \heatmapcolor{79.38}  & \heatmapcolor{83.04} & \heatmapcolor{86.58}  & \heatmapcolor{61.94} & \heatmapcolor{48.00}  & \heatmapcolor{63.90} \\
% \hline
% {\scriptsize Swin-B} &   \heatmapcolor{78.88} & \heatmapcolor{79.40} & \heatmapcolor{79.04}  & \heatmapcolor{86.60}  & \heatmapcolor{79.80}  & \heatmapcolor{81.22}  & \heatmapcolor{82.28}  & \heatmapcolor{81.48}  & \heatmapcolor{84.74} & \heatmapcolor{87.64}  & \heatmapcolor{66.82} & \heatmapcolor{68.28}  & \heatmapcolor{54.76} \\
% \hline

% \rowcolor{gray!5}
% \multicolumn{14}{|c|}{Projected Gradient Decent (PGD) at $\epsilon=\frac{8}{255}$} \\
% \hline
% {\scriptsize VSSM-T} &   \heatmapcolor{0.00}  & \heatmapcolor{37.26}  & \heatmapcolor{35.56}  & \heatmapcolor{81.44}  & \heatmapcolor{64.98}  & \heatmapcolor{76.84}  & \heatmapcolor{75.48}  & \heatmapcolor{82.58}  & \heatmapcolor{89.16}  & \heatmapcolor{91.80}  & \heatmapcolor{65.76} & \heatmapcolor{74.72} & \heatmapcolor{71.50}  \\
% \hline
% {\scriptsize VSSM-S} & \heatmapcolor{16.88} & \heatmapcolor{0.02} & \heatmapcolor{23.94} & \heatmapcolor{77.54} & \heatmapcolor{55.76} & \heatmapcolor{68.78} & \heatmapcolor{65.98} &\heatmapcolor{79.26} & \heatmapcolor{86.06} & \heatmapcolor{89.42} & \heatmapcolor{58.92} & \heatmapcolor{65.92} & \heatmapcolor{61.46}   \\
% \hline
% {\scriptsize VSSM-B} & \heatmapcolor{15.98} & \heatmapcolor{25.26} & \heatmapcolor{0.00} & \heatmapcolor{77.38} & \heatmapcolor{54.42} & \heatmapcolor{68.58} & \heatmapcolor{65.24} & \heatmapcolor{79.76} & \heatmapcolor{86.24} & \heatmapcolor{89.94} & \heatmapcolor{57.40} & \heatmapcolor{66.52} & \heatmapcolor{61.74}   \\
% \hline
% {\scriptsize ResNet-50} & \heatmapcolor{83.34} & \heatmapcolor{86.98} & \heatmapcolor{87.04} & \heatmapcolor{0.00} & \heatmapcolor{85.54} & \heatmapcolor{90.46} & \heatmapcolor{89.28} & \heatmapcolor{82.48} & \heatmapcolor{89.96} & \heatmapcolor{93.18} & \heatmapcolor{84.18} &\heatmapcolor{89.24} &\heatmapcolor{89.12}   \\
% \hline
% {\scriptsize ConvNext-T*} &  \heatmapcolor{73.74} & \heatmapcolor{78.36} & \heatmapcolor{76.62}  & \heatmapcolor{84.98}  & \heatmapcolor{0.00}  & \heatmapcolor{59.56}  & \heatmapcolor{67.00}  & \heatmapcolor{83.26}  & \heatmapcolor{88.06} & \heatmapcolor{91.48}  & \heatmapcolor{71.70} & \heatmapcolor{79.46}   & \heatmapcolor{78.16}  \\
% \hline
% {\scriptsize ConvNext-S*} &  \heatmapcolor{81.88} & \heatmapcolor{84.78} & \heatmapcolor{84.20}  & \heatmapcolor{88.42}  & \heatmapcolor{59.94}  & \heatmapcolor{0.00}  & \heatmapcolor{69.08}  & \heatmapcolor{84.94}  & \heatmapcolor{90.10} & \heatmapcolor{92.62}  & \heatmapcolor{77.08} & \heatmapcolor{83.00}  & \heatmapcolor{80.26}   \\
% \hline
% {\scriptsize ConvNext-B*} &  \heatmapcolor{69.56} & \heatmapcolor{73.62} & \heatmapcolor{72.22}  & \heatmapcolor{83.80}  & \heatmapcolor{50.48}  & \heatmapcolor{53.26}  & \heatmapcolor{0.00}  & \heatmapcolor{81.80}  & \heatmapcolor{86.90} & \heatmapcolor{89.58}  & \heatmapcolor{69.70} & \heatmapcolor{73.80}  & \heatmapcolor{70.72}    \\
% \hline
% {\scriptsize ViT-T} &   \heatmapcolor{92.10} & \heatmapcolor{93.82} & \heatmapcolor{94.26}  & \heatmapcolor{88.14}  & \heatmapcolor{91.30}  & \heatmapcolor{92.74}  & \heatmapcolor{92.90}  & \heatmapcolor{0.00}  & \heatmapcolor{55.58} & \heatmapcolor{77.34}  & \heatmapcolor{84.52} & \heatmapcolor{88.16}  & \heatmapcolor{89.24}  \\
% \hline
% {\scriptsize ViT-S} &    \heatmapcolor{87.28} & \heatmapcolor{89.34} & \heatmapcolor{89.70}  & \heatmapcolor{85.96}  & \heatmapcolor{85.66}  & \heatmapcolor{89.06}  & \heatmapcolor{88.48}  & \heatmapcolor{38.16}  & \heatmapcolor{0.00} & \heatmapcolor{48.68}  & \heatmapcolor{76.98} & \heatmapcolor{80.34} & \heatmapcolor{82.48}  \\
% \hline
% {\scriptsize ViT-B} &   \heatmapcolor{86.18} & \heatmapcolor{87.74} & \heatmapcolor{87.72}  & \heatmapcolor{85.04}  & \heatmapcolor{83.72}  & \heatmapcolor{86.64}  & \heatmapcolor{85.84}  & \heatmapcolor{53.50}  & \heatmapcolor{37.48} & \heatmapcolor{0.00}  & \heatmapcolor{77.02} & \heatmapcolor{79.56}  & \heatmapcolor{80.86}  \\
% \hline
% {\scriptsize Swin-T} &   \heatmapcolor{83.10} & \heatmapcolor{87.58} & \heatmapcolor{87.06}  & \heatmapcolor{89.58}  & \heatmapcolor{81.32}  & \heatmapcolor{85.24}  & \heatmapcolor{87.12}  & \heatmapcolor{83.32}  & \heatmapcolor{89.82} & \heatmapcolor{92.80}  & \heatmapcolor{0.00} & \heatmapcolor{39.00}  & \heatmapcolor{37.88}   \\
% \hline
% {\scriptsize Swin-S} &  \heatmapcolor{83.08} & \heatmapcolor{86.28} & \heatmapcolor{86.26}  & \heatmapcolor{89.76}  & \heatmapcolor{82.16}  & \heatmapcolor{85.82}  & \heatmapcolor{85.42}  & \heatmapcolor{82.96}  & \heatmapcolor{88.80} & \heatmapcolor{92.38}  & \heatmapcolor{25.40} & \heatmapcolor{0.00}  & \heatmapcolor{31.44}  \\
% \hline
% {\scriptsize Swin-B} &   \heatmapcolor{82.52} & \heatmapcolor{85.12} & \heatmapcolor{84.78}  & \heatmapcolor{89.88}  & \heatmapcolor{81.16}  & \heatmapcolor{83.38}  & \heatmapcolor{84.38}  & \heatmapcolor{84.24}  & \heatmapcolor{89.74} & \heatmapcolor{92.86}  & \heatmapcolor{27.30} & \heatmapcolor{34.36}  & \heatmapcolor{0.02}   \\
% \hline


% \end{tabular}
% }
% \vspace{-1em}

% \end{table}



% Above table is before updating table with convnext_1k results


\begin{table*}[t]
\centering
\caption{\small Robust accuracy of models under white-box and black-box settings for FGSM and PGD attacks. Adversarial examples  crafted on surrogate models are used to evaluate robustness of target models.}
\label{tab:adv_transf_main}
\setlength{\tabcolsep}{2.0pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{|l| c c c c c c c c c c c c c c c c|}
\hline
\rowcolor{LightCyan}
\multicolumn{1}{|l|}{\scriptsize Target $\rightarrow$} & \rotatebox{0}{\scriptsize \textbf{VMamba-T}} & \rotatebox{0}{\scriptsize \textbf{VMamba-S}} & \rotatebox{0}{\scriptsize \textbf{VMamba-B}} & \rotatebox{0}{\scriptsize \textbf{MambaVision-T}} & \rotatebox{0}{\scriptsize \textbf{MambaVision-S}} & \rotatebox{0}{\scriptsize \textbf{MambaVision-B}} & \rotatebox{0}{\scriptsize \textbf{ResNet-50}} & \rotatebox{0}{\scriptsize \textbf{ConvNext-T}} & \rotatebox{0}{\scriptsize \textbf{ConvNext-S}} & \rotatebox{0}{\scriptsize \textbf{ConvNext-B}} & \rotatebox{0}{\scriptsize \textbf{ViT-T}} & \rotatebox{0}{\scriptsize \textbf{ViT-S}} & \rotatebox{0}{\scriptsize \textbf{ViT-B}} & \rotatebox{0}{\scriptsize \textbf{Swin-T}} & \rotatebox{0}{\scriptsize \textbf{Swin-S}} & \rotatebox{0}{\scriptsize \textbf{Swin-B}} \\
\hline
\rowcolor{gray!5}
\multicolumn{1}{|l|}{\scriptsize Surrogate $\downarrow$} & \multicolumn{16}{c|}{Fast Gradient Sign Method (FGSM) at $\epsilon=\frac{8}{255}$ } \\
\hline
{\scriptsize VMamba-T} &   \heatmapcolor{42.90}  & \heatmapcolor{66.34}  & \heatmapcolor{65.10}  & \heatmapcolor{74.44}  & \heatmapcolor{73.00}  & \heatmapcolor{73.16}  & \heatmapcolor{80.20}  & \heatmapcolor{72.66}  & \heatmapcolor{73.80}  & \heatmapcolor{72.84}  & \heatmapcolor{79.46}  & \heatmapcolor{83.64}  & \heatmapcolor{86.94}  & \heatmapcolor{72.22} & \heatmapcolor{76.38} & \heatmapcolor{74.60}    \\
\hline
{\scriptsize VMamba-S} &  \heatmapcolor{62.24}  & \heatmapcolor{48.42}  & \heatmapcolor{63.00}  & \heatmapcolor{71.84}  & \heatmapcolor{71.92}  & \heatmapcolor{71.34}  & \heatmapcolor{79.70}  & \heatmapcolor{71.40}  & \heatmapcolor{71.04}  & \heatmapcolor{70.18}  & \heatmapcolor{78.42}  & \heatmapcolor{81.56}  & \heatmapcolor{84.58}  & \heatmapcolor{70.96}  & \heatmapcolor{72.92}  & \heatmapcolor{71.14}   \\
\hline
{\scriptsize VMamba-B} &   \heatmapcolor{65.52}  & \heatmapcolor{66.96}  & \heatmapcolor{51.24}  & \heatmapcolor{75.22}  & \heatmapcolor{73.82}  & \heatmapcolor{73.08}  & \heatmapcolor{81.22}  & \heatmapcolor{73.54}  & \heatmapcolor{73.20}  & \heatmapcolor{72.32}  & \heatmapcolor{79.12}  & \heatmapcolor{83.62}  & \heatmapcolor{86.24}  & \heatmapcolor{73.24}  & \heatmapcolor{76.30}  & \heatmapcolor{73.88} \\
\hline

{\scriptsize MambaVision-T} &   \heatmapcolor{77.74}  & \heatmapcolor{79.04}  & \heatmapcolor{79.78}   & \heatmapcolor{46.18}  & \heatmapcolor{73.30}  & \heatmapcolor{75.64} & \heatmapcolor{82.06}  & \heatmapcolor{79.50}  & \heatmapcolor{80.88}  & \heatmapcolor{81.82}  & \heatmapcolor{78.30}  & \heatmapcolor{84.20}  & \heatmapcolor{87.86}  & \heatmapcolor{77.78}  & \heatmapcolor{81.24}  & \heatmapcolor{80.80} \\
\hline

{\scriptsize MambaVision-S} &   \heatmapcolor{77.86}  & \heatmapcolor{79.56}  & \heatmapcolor{79.24}  & \heatmapcolor{74.96}  & \heatmapcolor{53.42}  & \heatmapcolor{73.84}  & \heatmapcolor{83.60}  & \heatmapcolor{80.40}  & \heatmapcolor{81.14}  & \heatmapcolor{81.26}  & \heatmapcolor{79.90}  & \heatmapcolor{85.64}  & \heatmapcolor{88.52}  & \heatmapcolor{78.50}  & \heatmapcolor{82.40}  & \heatmapcolor{81.88} \\
\hline

{\scriptsize MambaVision-B} &   \heatmapcolor{75.90}  & \heatmapcolor{77.84}  & \heatmapcolor{77.00}  & \heatmapcolor{75.46}  & \heatmapcolor{71.96}  & \heatmapcolor{52.68}  & \heatmapcolor{83.46}  & \heatmapcolor{80.24}  & \heatmapcolor{80.52}  & \heatmapcolor{79.92}  & \heatmapcolor{79.82}  & \heatmapcolor{85.18}  & \heatmapcolor{88.12}  & \heatmapcolor{78.46}  & \heatmapcolor{81.60}  & \heatmapcolor{80.30} \\
\hline

{\scriptsize ResNet-50} &   \heatmapcolor{81.38}  & \heatmapcolor{83.24}  & \heatmapcolor{83.84}  & \heatmapcolor{81.06}  & \heatmapcolor{82.54}  & \heatmapcolor{84.88}  & \heatmapcolor{30.46}  & \heatmapcolor{80.30}  & \heatmapcolor{82.20}  & \heatmapcolor{83.38}  & \heatmapcolor{75.94}  & \heatmapcolor{84.74}  & \heatmapcolor{89.12}  & \heatmapcolor{80.64}  & \heatmapcolor{85.00} & \heatmapcolor{85.42}  \\
\hline


% {\scriptsize ConvNext-T*} &  \heatmapcolor{72.78} & \heatmapcolor{75.20} & \heatmapcolor{74.26}  & \heatmapcolor{81.84}  & \heatmapcolor{37.14}  & \heatmapcolor{68.14}  & \heatmapcolor{69.96}  & \heatmapcolor{78.86}  & \heatmapcolor{82.56} & \heatmapcolor{84.96}  & \heatmapcolor{71.86} & \heatmapcolor{76.60}   & \heatmapcolor{74.96}  \\
% \hline


{\scriptsize ConvNext-T} &  \heatmapcolor{69.00} & \heatmapcolor{71.46} & \heatmapcolor{71.18}  & \heatmapcolor{73.50}  & \heatmapcolor{73.92}  & \heatmapcolor{74.40}  & \heatmapcolor{77.96}  & \heatmapcolor{36.36}  & \heatmapcolor{61.96}  & \heatmapcolor{63.76}  & \heatmapcolor{76.92}  & \heatmapcolor{82.74} & \heatmapcolor{85.58}  & \heatmapcolor{67.06} & \heatmapcolor{71.88}   & \heatmapcolor{70.78}  \\
\hline




% {\scriptsize ConvNext-S*} &  \heatmapcolor{81.16} & \heatmapcolor{82.92} & \heatmapcolor{81.66}  & \heatmapcolor{86.14}  & \heatmapcolor{74.40}  & \heatmapcolor{54.28}  & \heatmapcolor{75.12}  & \heatmapcolor{82.44}  & \heatmapcolor{85.74} & \heatmapcolor{87.20}  & \heatmapcolor{79.32} & \heatmapcolor{82.40}  & \heatmapcolor{80.70}  \\
% \hline


{\scriptsize ConvNext-S} &  \heatmapcolor{69.54} & \heatmapcolor{70.62} & \heatmapcolor{70.48}  & \heatmapcolor{74.68}  & \heatmapcolor{74.38}  & \heatmapcolor{75.24}  & \heatmapcolor{79.48}  & \heatmapcolor{63.48}  & \heatmapcolor{49.10}  & \heatmapcolor{63.62}  & \heatmapcolor{78.48}  & \heatmapcolor{82.94} & \heatmapcolor{85.02}  & \heatmapcolor{69.24} & \heatmapcolor{71.54}  & \heatmapcolor{69.74}  \\
\hline


% {\scriptsize ConvNext-B*} &  \heatmapcolor{75.94} & \heatmapcolor{76.80} & \heatmapcolor{76.18}  & \heatmapcolor{83.26}  & \heatmapcolor{68.98}  & \heatmapcolor{69.30}  & \heatmapcolor{45.42}  & \heatmapcolor{79.02}  & \heatmapcolor{82.36} & \heatmapcolor{83.74}  & \heatmapcolor{75.60} & \heatmapcolor{76.80}  & \heatmapcolor{75.82}   \\
% \hline


{\scriptsize ConvNext-B} &  \heatmapcolor{70.54} & \heatmapcolor{71.78} & \heatmapcolor{69.78}  & \heatmapcolor{76.78}  & \heatmapcolor{75.02}  & \heatmapcolor{74.82}  & \heatmapcolor{81.72}  & \heatmapcolor{67.34}  & \heatmapcolor{66.24}  & \heatmapcolor{51.32}  & \heatmapcolor{80.26}  & \heatmapcolor{83.98} & \heatmapcolor{86.22}  & \heatmapcolor{69.86} & \heatmapcolor{73.44}  & \heatmapcolor{70.84}   \\
\hline




{\scriptsize ViT-T} &   \heatmapcolor{85.92} & \heatmapcolor{88.30} & \heatmapcolor{88.88}  & \heatmapcolor{82.16}  & \heatmapcolor{85.06}  & \heatmapcolor{87.24}  & \heatmapcolor{82.68}  & \heatmapcolor{85.08}  & \heatmapcolor{86.56}  & \heatmapcolor{88.06}  & \heatmapcolor{2.28}  & \heatmapcolor{50.04} & \heatmapcolor{69.90}  & \heatmapcolor{75.66} & \heatmapcolor{79.72}  & \heatmapcolor{82.32}  \\
\hline
{\scriptsize ViT-S} &    \heatmapcolor{81.74} & \heatmapcolor{83.76} & \heatmapcolor{84.46}  & \heatmapcolor{78.94}  & \heatmapcolor{80.78}  & \heatmapcolor{82.68}  & \heatmapcolor{81.70}  & \heatmapcolor{82.34}  & \heatmapcolor{82.78}  & \heatmapcolor{84.38}  & \heatmapcolor{45.40}  & \heatmapcolor{11.02} & \heatmapcolor{54.82}  & \heatmapcolor{72.50} & \heatmapcolor{75.98} & \heatmapcolor{77.88}  \\
\hline
{\scriptsize ViT-B} &    \heatmapcolor{82.46} & \heatmapcolor{84.02} & \heatmapcolor{84.48}  & \heatmapcolor{80.40}  & \heatmapcolor{81.82}  & \heatmapcolor{82.46}  & \heatmapcolor{81.90}  & \heatmapcolor{82.04}  & \heatmapcolor{82.24}  & \heatmapcolor{83.62}  & \heatmapcolor{58.50}  & \heatmapcolor{53.84} & \heatmapcolor{24.24}  & \heatmapcolor{75.82} & \heatmapcolor{77.62}  & \heatmapcolor{78.54} \\
\hline
{\scriptsize Swin-T} &    \heatmapcolor{72.40} & \heatmapcolor{76.06} & \heatmapcolor{75.58}  & \heatmapcolor{76.80}  & \heatmapcolor{77.16}  & \heatmapcolor{78.06}  & \heatmapcolor{82.82}  & \heatmapcolor{71.46}  & \heatmapcolor{72.12}  & \heatmapcolor{71.96}  & \heatmapcolor{76.48}  & \heatmapcolor{80.66} & \heatmapcolor{85.46}  & \heatmapcolor{28.86} & \heatmapcolor{56.22}  & \heatmapcolor{55.12}  \\
\hline
{\scriptsize Swin-S} &   \heatmapcolor{78.24} & \heatmapcolor{79.10} & \heatmapcolor{79.30}  & \heatmapcolor{80.12}  & \heatmapcolor{81.90}  & \heatmapcolor{81.40}  & \heatmapcolor{85.46}  & \heatmapcolor{77.96}  & \heatmapcolor{77.10}  & \heatmapcolor{77.02}  & \heatmapcolor{79.38}  & \heatmapcolor{83.04} & \heatmapcolor{86.58}  & \heatmapcolor{61.94} & \heatmapcolor{48.00}  & \heatmapcolor{63.90} \\
\hline
{\scriptsize Swin-B} &   \heatmapcolor{78.88} & \heatmapcolor{79.40} & \heatmapcolor{79.04}  & \heatmapcolor{81.48}  & \heatmapcolor{82.16}  & \heatmapcolor{81.04}  & \heatmapcolor{86.60}  & \heatmapcolor{78.16}  & \heatmapcolor{78.46}  & \heatmapcolor{77.32}  & \heatmapcolor{81.48}  & \heatmapcolor{84.74} & \heatmapcolor{87.64}  & \heatmapcolor{66.82} & \heatmapcolor{68.28}  & \heatmapcolor{54.76} \\
\hline

\rowcolor{gray!5}
\multicolumn{16}{|c|}{Projected Gradient Decent (PGD) at $\epsilon=\frac{8}{255}$} \\
\hline
{\scriptsize VMamba-T} &   \heatmapcolor{0.00}  & \heatmapcolor{37.26}  & \heatmapcolor{35.56}  & \heatmapcolor{70.86}  & \heatmapcolor{67.72}  & \heatmapcolor{68.78}  & \heatmapcolor{81.44}  & \heatmapcolor{63.54}  & \heatmapcolor{67.18}  & \heatmapcolor{65.88}  & \heatmapcolor{82.58}  & \heatmapcolor{89.16}  & \heatmapcolor{91.80}  & \heatmapcolor{65.76} & \heatmapcolor{74.72} & \heatmapcolor{71.50}  \\
\hline
{\scriptsize VMamba-S} & \heatmapcolor{16.88} & \heatmapcolor{0.02} & \heatmapcolor{23.94}  & \heatmapcolor{60.98}  & \heatmapcolor{60.22}  & \heatmapcolor{59.16} & \heatmapcolor{77.54} & \heatmapcolor{56.24} & \heatmapcolor{57.72} & \heatmapcolor{56.16} &\heatmapcolor{79.26} & \heatmapcolor{86.06} & \heatmapcolor{89.42} & \heatmapcolor{58.92} & \heatmapcolor{65.92} & \heatmapcolor{61.46}   \\
\hline
{\scriptsize VMamba-B} & \heatmapcolor{15.98} & \heatmapcolor{25.26} & \heatmapcolor{0.00}  & \heatmapcolor{64.56}  & \heatmapcolor{59.68}  & \heatmapcolor{59.34} & \heatmapcolor{77.38} & \heatmapcolor{56.30} & \heatmapcolor{57.94} & \heatmapcolor{53.42} & \heatmapcolor{79.76} & \heatmapcolor{86.24} & \heatmapcolor{89.94} & \heatmapcolor{57.40} & \heatmapcolor{66.52} & \heatmapcolor{61.74}   \\
\hline

{\scriptsize MambaVision-T} &   \heatmapcolor{76.62}  & \heatmapcolor{79.98}  & \heatmapcolor{80.92}  & \heatmapcolor{0.00}  & \heatmapcolor{64.18}  & \heatmapcolor{71.78}  & \heatmapcolor{85.76}  & \heatmapcolor{80.04}  & \heatmapcolor{82.50}  & \heatmapcolor{84.24}  & \heatmapcolor{82.62}  & \heatmapcolor{88.90}  & \heatmapcolor{92.46}  & \heatmapcolor{78.86}  & \heatmapcolor{83.42}  & \heatmapcolor{83.14} \\
\hline

{\scriptsize MambaVision-S} &   \heatmapcolor{67.52}  & \heatmapcolor{73.60}  & \heatmapcolor{71.86}  & \heatmapcolor{55.92}  & \heatmapcolor{0.00}  & \heatmapcolor{53.36}  & \heatmapcolor{83.72}  & \heatmapcolor{74.72}  & \heatmapcolor{78.04}  & \heatmapcolor{77.26}  & \heatmapcolor{82.18}  & \heatmapcolor{88.88}  & \heatmapcolor{91.68}  & \heatmapcolor{74.60}  & \heatmapcolor{81.44}  & \heatmapcolor{79.64} \\
\hline

{\scriptsize MambaVision-B} &   \heatmapcolor{62.06}  & \heatmapcolor{67.32}  & \heatmapcolor{65.76}  & \heatmapcolor{58.66}  & \heatmapcolor{47.54}  & \heatmapcolor{0.12}  & \heatmapcolor{83.20}  & \heatmapcolor{72.80}  & \heatmapcolor{75.38}  & \heatmapcolor{73.28}  & \heatmapcolor{82.18}  & \heatmapcolor{87.94}  & \heatmapcolor{91.00}  & \heatmapcolor{72.04}  & \heatmapcolor{77.78}  & \heatmapcolor{75.60} \\
\hline

{\scriptsize ResNet-50} & \heatmapcolor{83.34} & \heatmapcolor{86.98} & \heatmapcolor{87.04} & \heatmapcolor{83.96}  & \heatmapcolor{85.56}  & \heatmapcolor{87.82}  & \heatmapcolor{0.00} & \heatmapcolor{81.00} & \heatmapcolor{84.92} & \heatmapcolor{86.30} & \heatmapcolor{82.48} & \heatmapcolor{89.96} & \heatmapcolor{93.18} & \heatmapcolor{84.18} &\heatmapcolor{89.24} &\heatmapcolor{89.12}   \\
\hline

% {\scriptsize ConvNext-T*} &  \heatmapcolor{73.74} & \heatmapcolor{78.36} & \heatmapcolor{76.62}  & \heatmapcolor{84.98}  & \heatmapcolor{0.00}  & \heatmapcolor{59.56}  & \heatmapcolor{67.00}  & \heatmapcolor{83.26}  & \heatmapcolor{88.06} & \heatmapcolor{91.48}  & \heatmapcolor{71.70} & \heatmapcolor{79.46}   & \heatmapcolor{78.16}  \\
% \hline

{\scriptsize ConvNext-T} &  \heatmapcolor{60.58} & \heatmapcolor{67.06} & \heatmapcolor{66.48}  & \heatmapcolor{73.34}  & \heatmapcolor{73.46}  & \heatmapcolor{76.26}  & \heatmapcolor{79.76}  & \heatmapcolor{0.00}  & \heatmapcolor{31.32}  & \heatmapcolor{39.70}  & \heatmapcolor{80.44}  & \heatmapcolor{87.28} & \heatmapcolor{90.46}  & \heatmapcolor{56.02} & \heatmapcolor{66.62}   & \heatmapcolor{64.40}  \\
\hline





% {\scriptsize ConvNext-S*} &  \heatmapcolor{81.88} & \heatmapcolor{84.78} & \heatmapcolor{84.20}  & \heatmapcolor{88.42}  & \heatmapcolor{59.94}  & \heatmapcolor{0.00}  & \heatmapcolor{69.08}  & \heatmapcolor{84.94}  & \heatmapcolor{90.10} & \heatmapcolor{92.62}  & \heatmapcolor{77.08} & \heatmapcolor{83.00}  & \heatmapcolor{80.26}   \\
% \hline

{\scriptsize ConvNext-S} &  \heatmapcolor{58.04} & \heatmapcolor{63.20} & \heatmapcolor{62.96}  & \heatmapcolor{71.40}  & \heatmapcolor{71.80}  & \heatmapcolor{74.20}   & \heatmapcolor{78.22}  & \heatmapcolor{24.96}  & \heatmapcolor{0.00}  & \heatmapcolor{33.96}  & \heatmapcolor{80.02}  & \heatmapcolor{86.20} & \heatmapcolor{89.86}  & \heatmapcolor{52.70} & \heatmapcolor{62.58}  & \heatmapcolor{60.54}   \\
\hline





% {\scriptsize ConvNext-B*} &  \heatmapcolor{69.56} & \heatmapcolor{73.62} & \heatmapcolor{72.22}  & \heatmapcolor{83.80}  & \heatmapcolor{50.48}  & \heatmapcolor{53.26}  & \heatmapcolor{0.00}  & \heatmapcolor{81.80}  & \heatmapcolor{86.90} & \heatmapcolor{89.58}  & \heatmapcolor{69.70} & \heatmapcolor{73.80}  & \heatmapcolor{70.72}    \\
% \hline


{\scriptsize ConvNext-B} &  \heatmapcolor{58.24} & \heatmapcolor{64.04} & \heatmapcolor{60.40}  & \heatmapcolor{75.86}  & \heatmapcolor{73.96}  & \heatmapcolor{73.88}  & \heatmapcolor{80.80}  & \heatmapcolor{35.84}  & \heatmapcolor{36.60}  & \heatmapcolor{0.00}  & \heatmapcolor{81.48}  & \heatmapcolor{87.22} & \heatmapcolor{90.36}  & \heatmapcolor{51.80} & \heatmapcolor{63.16}  & \heatmapcolor{58.62}    \\
\hline




{\scriptsize ViT-T} &   \heatmapcolor{92.10} & \heatmapcolor{93.82} & \heatmapcolor{94.26}  & \heatmapcolor{89.58}  & \heatmapcolor{91.46}  & \heatmapcolor{93.44}  & \heatmapcolor{88.14}  & \heatmapcolor{90.44}  & \heatmapcolor{92.18}  & \heatmapcolor{93.28}  & \heatmapcolor{0.00}  & \heatmapcolor{55.58} & \heatmapcolor{77.34}  & \heatmapcolor{84.52} & \heatmapcolor{88.16}  & \heatmapcolor{89.24}  \\
\hline
{\scriptsize ViT-S} &    \heatmapcolor{87.28} & \heatmapcolor{89.34} & \heatmapcolor{89.70}  & \heatmapcolor{83.78}  & \heatmapcolor{87.16}  & \heatmapcolor{88.68}  & \heatmapcolor{85.96}  & \heatmapcolor{86.34}  & \heatmapcolor{87.90}  & \heatmapcolor{89.26}  & \heatmapcolor{38.16}  & \heatmapcolor{0.00} & \heatmapcolor{48.68}  & \heatmapcolor{76.98} & \heatmapcolor{80.34} & \heatmapcolor{82.48}  \\
\hline
{\scriptsize ViT-B} &   \heatmapcolor{86.18} & \heatmapcolor{87.74} & \heatmapcolor{87.72}  & \heatmapcolor{83.22}  & \heatmapcolor{85.58}  & \heatmapcolor{87.18}  & \heatmapcolor{85.04}  & \heatmapcolor{85.56}  & \heatmapcolor{86.10}  & \heatmapcolor{87.62}  & \heatmapcolor{53.50}  & \heatmapcolor{37.48} & \heatmapcolor{0.00}  & \heatmapcolor{77.02} & \heatmapcolor{79.56}  & \heatmapcolor{80.86}  \\
\hline
{\scriptsize Swin-T} &   \heatmapcolor{83.10} & \heatmapcolor{87.58} & \heatmapcolor{87.06}  & \heatmapcolor{86.98}  & \heatmapcolor{88.18}  & \heatmapcolor{89.60}  & \heatmapcolor{89.58}  & \heatmapcolor{79.30}  & \heatmapcolor{81.52}  & \heatmapcolor{80.28}  & \heatmapcolor{83.32}  & \heatmapcolor{89.82} & \heatmapcolor{92.80}  & \heatmapcolor{0.00} & \heatmapcolor{39.00}  & \heatmapcolor{37.88}   \\
\hline
{\scriptsize Swin-S} &  \heatmapcolor{83.08} & \heatmapcolor{86.28} & \heatmapcolor{86.26}  & \heatmapcolor{85.86}  & \heatmapcolor{88.22}  & \heatmapcolor{88.74}  & \heatmapcolor{89.76}  & \heatmapcolor{79.60}  & \heatmapcolor{80.68}  & \heatmapcolor{79.84}  & \heatmapcolor{82.96}  & \heatmapcolor{88.80} & \heatmapcolor{92.38}  & \heatmapcolor{25.40} & \heatmapcolor{0.00}  & \heatmapcolor{31.44}  \\
\hline
{\scriptsize Swin-B} &   \heatmapcolor{82.52} & \heatmapcolor{85.12} & \heatmapcolor{84.78}  & \heatmapcolor{86.86}  & \heatmapcolor{88.02}  & \heatmapcolor{88.68}  & \heatmapcolor{89.88}  & \heatmapcolor{79.18}  & \heatmapcolor{80.08}  & \heatmapcolor{78.92}  & \heatmapcolor{84.24}  & \heatmapcolor{89.74} & \heatmapcolor{92.86}  & \heatmapcolor{27.30} & \heatmapcolor{34.36}  & \heatmapcolor{0.02}   \\
\hline


\end{tabular}
}
\vspace{-0em}

\end{table*}




